TGB 2.0: A Benchmark for Learning on Temporal Knowledge Graphs and Heterogeneous Graphs

Multi-relational temporal graphs are powerful tools for modeling real-world data, capturing the evolving and interconnected nature of entities over time. Recently, many novel models are proposed for ML on such graphs intensifying the need for robust evaluation and standardized benchmark datasets. However, the availability of such resources remains scarce and evaluation faces added complexity due to reproducibility issues in experimental protocols. To address these challenges, we introduce Temporal Graph Benchmark 2.0 (TGB 2.0), a novel benchmarking framework tailored for evaluating methods for predicting future links on Temporal Knowledge Graphs and Temporal Heterogeneous Graphs with a focus on large-scale datasets, extending the Temporal Graph Benchmark. TGB 2.0 facilitates comprehensive evaluations by presenting eight novel datasets spanning five domains with up to 53 million edges. TGB 2.0 datasets are significantly larger than existing datasets in terms of number of nodes, edges, or timestamps. In addition, TGB 2.0 provides a reproducible and realistic evaluation pipeline for multi-relational temporal graphs. Through extensive experimentation, we observe that 1) leveraging edge-type information is crucial to obtain high performance, 2) simple heuristic baselines are often competitive with more complex methods, 3) most methods fail to run on our largest datasets, highlighting the need for research on more scalable methods.

==> chapters/01_introduction.tex <==
\label{sec:introduction}
% multirelational temporal graphs are cool
% Many approaches have been proposed in recent years for predicting future links in multirelations temporal graph
% When it comes to evaluation these approaches, we found some issues: 
%% inconsistencies in evaluation
%% comparison to baselines
%% evaluation is mostly done on small-scale datasets
%in this work, we tackle the above isses by presenting \name

% A) multirelational graphs are cool and many approaches have been proposed
%\ah{[added a little more background]}. 
% \er{These works on molecular graphs are not doing link prediction, right?}
Learning from graph-structured data has become ubiquitous in many applications such as recommendation systems~\cite{kumar2019predicting,wu2022graph}, knowledge base completion~\cite{nickel2015review,liu2021indigo} and molecular learning~\cite{rampavsek2022recipe,beaini2023towards}. Relational data often evolves over time and can contain multiple types of relations. These complex interactions and temporal dependencies can be captured by \textit{multi-relational} temporal graphs. In recent years, various approaches have emerged to predict future links in such graphs, notably for prediction on Temporal Knowledge Graphs (TKGs)~\cite{Li2021regcn,Liu2021tlogic} and Temporal Heterogeneous Graphs (THGs)~\cite{li2023simplifying,ji2021dynamic}.
These approaches capture the rich information from multi-relational data, forming distinct lines of research from those of single-relational temporal graphs~\cite{rossi2020temporal,luo2022neighborhood}. However, benchmarking on multi-relational temporal graphs faces two main challenges: \emph{inconsistent evaluation} and \emph{limited dataset size}.
%To capture the rich information from multi-relational data, specialized TKG and THG methods varies significantly from that of the single-relational temporal graph methods~\cite{rossi2020temporal,} thus forming novel lines of research. 

%Multi-relational temporal graphs are increasingly recognized as a powerful way of modeling dynamic systems, capturing complex interactions and temporal dependencies across diverse domains.

%A variety of ML approaches has been proposed for multi-relational temporal graphs, for both, Temporal Knowledge Graphs, as well as Temporal Heterogeneous Graphs.
%\subsection{Current Issues}
%\begin{itemize}
%    \item Recently it was found that a lot of inconsistencies exist in the evaluation of TKG models. 
%    \item Further, a simple baseline can beat existing TKG forecasting models on multiple datasets.
%    \item No large-scale datasets exist for TKG forecasting (What about THG?)
%    \item All in all, this leads to the fact that models are hard to compare, progress in the field is hard to grasp, and models are developed not with a focus on scalability to large-scale tasks.
%\end{itemize}
\begin{figure}[t]
\begin{subfigure}{0.47\textwidth}
\centering
 \includegraphics[width=\textwidth]{img/dataset_statstkg.pdf}
  \caption{Novel Temporal Knowledge Graphs} \label{fig:dataoldnewtkg}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/dataset_statsthg.pdf}
  \caption{Novel Temporal Heterogeneous Graphs} \label{fig:dataoldnewthg}
\end{subfigure}%

\caption{Existing benchmark datasets~(yellow) vs. novel datasets in \name for TKG (a) marked in \tkgdata{orange}   %\textcolor{orange}\tkgdata{orange} 
and THG (b) marked in \thgdata{green}. %\textcolor{green}{green}. 
Circle sizes correspond to the number of timestamps. \name datasets are significantly larger than existing datasets in number of nodes, edges and timestamps.}
 \label{fig:dataoldnew}
\vskip -0.3in
% \vspace{-1em}
\end{figure}

% B) issues with evaluation
%\ah{discuss the limitations in more details here and add more citations to back it up.}
%However, the evaluation of these approaches presents several challenges, including inconsistencies such as computing scores with different filter settings, comparing models for in multi-step prediction setting to models in single-step prediction setting, and different dataset versions~\cite{gastinger2023eval}. 
%Similar inconsistencies in evaluation have been observed in related research fields such as link prediction on Static Knowledge Graphs~\cite{Sun2020reevaluation,rossi2021knowledge}, node and graph classification on static graphs~\cite{shchur_pitfalls_2018,errica_fair_2020}, and temporal single-relational graph learning~\cite{huang2023temporal}.

\textbf{Inconsistent Evaluation.} Evaluation for multi-relational temporal graphs faces significant challenges. Recently, it was shown that existing evaluation for TKGs has inconsistencies in a) the evaluation metrics, % static filtered mrr vs temporal filtered mrr vs raw mrr
b) mixing multi-step and single-step prediction settings and c) using different versions of the same dataset ~\cite{gastinger2023eval}. Similar inconsistencies have been observed in related areas such as link prediction on static knowledge graphs~\cite{Sun2020reevaluation,rossi2021knowledge}, node and graph classification on static graphs~\cite{shchur_pitfalls_2018,errica_fair_2020}, and temporal graph link prediction~\cite{huang2023temporal}. In addition, for link prediction on THGs, existing evaluation often includes a single random negative per positive edge~\cite{li2023simplifying,xue2021modeling}, leading to over-optimistic performances, inconsistent evaluation, and reducing performance differentiation between methods~\cite{poursafaei2022edgebank}.

%that can be extended with new methods in the future, will help facilitate fair comparison between methods. 

% Furthermore, recent work also highlights the need to compare against simple baselines on evolving networks~\cite{gastinger2024baselines,poursafaei2022edgebank}. 
% Furthermore, recent work~\cite{gastinger2024baselines} highlights issues related to the limited or non-existent comparison to baselines, a problem previously also found in static Knowledge Graph completion, where simple rule-based systems can outperform embedding-based ones \cite{meilicke2018fine}, and in single-relational static and temporal graph tasks where structure-agnostic baselines compete with deep graph networks~\cite{poursafaei2022edgebank,errica2023class}.

\textbf{Limited Dataset Size.} Existing evaluations are conducted on predominantly small-scale datasets. For example, commonly used TKG and THG datasets consist of less than two million edges and one million nodes~\cite{li2023simplifying,ji2021dynamic,Li2021regcn,Li2022cen}. However, real world networks typically contain tens of millions of nodes and edges thus existing datasets rarely reflect the true scale of datasets in practice. In addition, significant efforts were made to design scalable graph learning methods for real applications which requires the availability of large scale datasets~\cite{Hu2020ogb,OGB_LSC,huang2023temporal}. These challenges hinder meaningful comparisons between methods and the accurate assessment of progress, and hamper advancements in the field. Therefore, there is an urgent need for a public and standardized benchmark to facilitate proper and fair comparison between methods, accelerating research for multi-relational temporal graphs.

% Thus, the availability of a public and reproducible evaluation pipeline will facilitate fair comparison between methods and accelerate research for multi-relational temporal graphs. 

% and pose obstacles to the development of scalable solutions for large-scale tasks. 



% C) how we tackle these issues and what is tgb
%In response to these challenges, we present \name, a benchmarking framework designed for evaluating methods for future link prediction on both TKG and THG.  Building upon the foundations laid by the Open Graph Benchmark (OGB)~\cite{Hu2020ogb}, which focuses on static graphs, and the Temporal Graph Benchmark (TGB)~\cite{Huang2023tgb}, which focuses on single-relational temporal graphs, \name extends TGB's capabilities to incorporate multi-relational temporal graphs. 
%\ah{[rephrasing the paragraph]}
%To address the aforementioned limitations, we present \name, extending the Temporal Graph Benchmark~\cite{Huang2023tgb} to multi-relational temporal graphs including TKGs and THGs.  

%Building upon the foundations laid by the Open Graph Benchmark (OGB)~\cite{Hu2020ogb}, GraphWorld~\cite{palowitch2022graphworld}, and OGB Large-Scale Challenge~\cite{OGB_LSC}, which focus on static graphs, and the Temporal Graph Benchmark (TGB)~\cite{Huang2023tgb}, which focuses on single-relational temporal graphs, \name extends TGB's capabilities to incorporate \emph{multi-relational temporal graphs} including TKGs and THGs. 
%The x-axis and y-axis of the plots shows the number of nodes and edges in the graph where the circle sizes indicate the number of timestamps. 
To address the aforementioned challenges, we present \name, a novel benchmark designed for future link prediction on multi-relational temporal graphs. Building upon the foundations of the Temporal Graph Benchmark (TGB)~\cite{Huang2023tgb} where only  \emph{single-relation temporal graphs} are included, \name introduces \emph{multi-relational temporal graph} datasets. 
\name adds four novel TKG datasets and four novel THG datasets of varying scale, spanning five domains. Figure~\ref{fig:dataoldnew} shows the difference in scale of the novel datasets in \name when compared to existing ones. Figure~\ref{fig:dataoldnewtkg} shows that \name TKG datasets (marked in orange) are orders of magnitude larger than existing ones in terms of number of nodes, edges and timestamps. Figure~\ref{fig:dataoldnewthg} shows that \name THG datasets (marked in green) are significantly larger than existing datasets, with \myket dataset quintupling the number of edges and timestamps, while \github has the most number of nodes to date.
Additionally, \name provides an automated evaluation pipeline for reproducible and realistic evaluation on multi-relational temporal graphs. In \name, the dynamic link property prediction task is treated as a ranking problem where multiple negative edges are ranked against the positive edge. For large datasets, we sample negative edges based on the edge type of the query, and thus closely approximate the complete evaluation where all negative edges are used. Overall, \name presents a benchmark for realistic, challenging, and reproducible evaluation on \emph{multi-relational temporal graphs} while providing an automated pipeline for dataset downloading, processing, evaluation as well as a public leaderboard.  %The evaluation mitigates temporal conflicts while sampling challenging negatives for each edge type where needed (\fp{this sentence is unclear to me.}). 
%Similarly, Figure~\ref{fig:dataoldnewthg} shows that \name datasets are larger than existing THG datasets as well. 
% Additionally, \name introduces a standardized evaluation pipeline, encompassing evaluation protocols tailored for both smaller and larger datasets, 
% mitigating temporal conflicts, and addressing the inherent challenges of multi-relational graphs.  
% Overall, \name facilitates a comprehensive evaluation of machine learning methods on multi-relational temporal graphs, ensuring realism, reproducibility, and robustness in the assessment process. Similar to OGB and TGB, \name features dataset acquisition, processing, and evaluation protocols, and is accompanied by a public leaderboard for model comparisons.
% \ah{TGB doesn't include any heterogenous graph and knowledge graph, explain our novel contribution in comparison.}
% \ah{It is important to have knowledge graph, it is usually requires different methods and line of research it is important to incorporate.}
%% C2) evaluation pipeline
% \name facilitates a comprehensive evaluation of machine learning methods on multi-relational temporal graphs, ensuring realism, reproducibility, and robustness in the assessment process. Similar to OGB and TGB, \name features dataset acquisition, processing, and evaluation protocols, and is accompanied by a public leaderboard for model comparisons.
% %% C1) datasets
% In this work, we introduce novel multi-relational datasets curated for TKG and THG forecasting tasks. These datasets are notably larger than existing ones, facilitating the exploration of long-range temporal dependencies and the development of more scalable methods. 
% %% C2) evaluation pipeline
% Additionally, we present a standardized evaluation pipeline, encompassing metrics tailored for both smaller and larger datasets, mitigating temporal conflicts and addressing the inherent challenges of multi-relational graphs.  
%For the smaller datasets, we compute the time-filtered Mean Reciprocal Rank (MRR) to evaluate methods. For larger datasets, we sample a fixed amount of negative samples per positive sample, where we use a destination-aware approach for TKG, and a node-type aware approach for THG and ensure to avoid temporal conflicts.
%\subsection{This work}
%In this work we present \name, a benchmarking framework designed for evaluating methods for future link prediction on Temporal Knowledge Graphs and Temporal Heterogeneous Graphs.
%It extends the capabilities of the Temporal Graph Benchmark (TGB), which primarily focuses on single-relational graphs, by incorporating multi-relational capabilities. 
%This extension enables a comprehensive evaluation of machine learning methods on multi-relational temporal graphs, ensuring realism, reproducibility, and robustness in the assessment process. 
%Much like OGB and TGB, \name features dataset acquisition, processing, and evaluation protocols, and offers a public leaderboard for model comparisons. 
%In this work we introduce \textit{new multi-relational datasets} as well as \textit{evaluation protocols} specifically tailored for multi-relational temporal graphs. This enhances its utility in assessing performance across Temporal Knowledge Graphs and Temporal Heterogeneous Graph Forecasting tasks.
% D) what are our contributions
%Our contributions include the provision of large and diverse datasets for multi-relational graphs, a unified evaluation framework, and a public leaderboard for method comparison. 
%\subsection{Contribution}
\name has the following main contributions:
\begin{itemize}[leftmargin=*]%[left=0pt]
 \item \textbf{Large and diverse datasets for multi-relational graphs.} We present four novel TKGs that are orders of magnitude larger than existing ones and four novel THGs that are significantly larger in number of nodes, edges and timestamps when compared with current ones. 
 % We present a total of eight novel multi-relational temporal graphs from five distinct domains. \name datasets are significantly larger than existing ones in number of nodes, edges and timestamps. 

\item \textbf{Realistic and reproducible evaluation.} We provide an evaluation pipeline for multi-relational temporal graphs, which automates the dataset downloading, processing and benchmarking process for seamless reproducibility. \name evaluation uses the ranking metric MRR and samples challenging negative edges based on the edge type information, hence providing realistic evaluation. 
% \item \textbf{Unified evaluation and public leaderboard.} We provide an automated and reproducible evaluation pipeline for multi-relational temporal graphs, extending the TGB framework to TKGs and THGs. A public leaderboard is also presented to track the recent progress in the field.
 
% \item \textbf{Unified evaluation and public leaderboard.} We provide a standardized evaluation pipeline by extending the automated and reproducible pipeline from TGB to integrate multi-relational temporal graphs. A public leaderboard is also presented to track the recent progress in the field.

% This does not only provide the possibility for reproducing our results, but also gives the possibility for researchers to include methods for their own new methods.
\item \textbf{Experimental insights.} The main insight from our experiments is that for both THGs and TKGs, all methods (apart from heuristics) fail to scale to our largest datasets, highlighting the need for more research on scalable methods. Surprisingly, the heuristic baselines perform competitively with more sophisticated methods. On THG datasets, we observe that methods that leverage the edge type and node type information achieve strong performance. Finally, across TKG datasets, we observe a strong correlation between the recurrency degree of a given relation type and the performance of methods, suggesting large room for improvement on  low recurrency relations.  
% highlighting scalability as a promising direction. 

% Through extensive experiments, we provide insights into the performance of existing methods and lay the foundation for future advancements in the field of TKG and THG learning. %We show \todo{insights from experiments todo} . %   \item (benchmark) How well does exciting methods work? What are the limitations? Do they scale? Do they work across datasets domains, if not, why? 
%    \item (realistics new tasks) churn prediction on temporal heterogeneous graph and (? duration prediction for temporal knowledge graph )
\end{itemize} 

\textbf{Reproducibility.} \name code and datasets are publicly available (see Appendix~\ref{app:datasetdoc} for download links) and the\href{https://tgb.complexdatalab.com/}{\name website} provides detailed documentation. 

%on \href{https://github.com/JuliaGast/TGB2}{Github} (details see Appendix~\ref{app:datasetdoc}). 



% \todo{Reproducibility: TGB code, datasets, leaderboards and details are on the TGB website. The code is
% also publicly available on GitHub with documentations seen here.}





==> chapters/10_acknowledgement.tex <==
% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
% \end{ack}



% \begin{ack}
% We thank the OGB team for providing the data mining script examples for the Wikidata. We thank Jacob Danovitch for setting up the public data upload in TGB which we continue to use here.

% \todo{ANDY: original tgb authors; compute canada stuff and data hosting, also "This research was enabled in part by compute resources, software and technical help provided by Mila (mila.quebec)."}
% \end{ack}

==> chapters/preliminaries/02_Preliminaries.tex <==
\subsection{Temporal Knowledge Graphs: Definition}
(\textit{Text in this section copied from \cite{gastinger2024baselines}})

 A \textit{Temporal Knowledge Graph} \G  is a set of quadruples $(s,r,o,t)$ with $s, o \in E$, relation $r \in R$, and time stamp $t \in T$ with $T = \{ 1 \ldots n \}, n \in \mathbb{N}^+$. More precisely, $E$ is the set of entities, $R$ is the set of possible relations, and $T$ is the set of timesteps. 
 A quadruple's $(s,r,o,t)$ semantic meaning is that $s$ is in relation $r$ to $o$ at $t$. % or during $t$.
 Alternatively, we may refer to this quadruple as a temporal triple that holds during the timestep $t$.

\subsection{Temporal Heterogeneous Graphs: Definition}
\textcolor{red}{TODO}

\subsection{TKG vs THG}
Heterogeneous graphs are those who have different node types and might be multi-partite, that is, there are no edges between nodes of the same type. Examples of heterogeneous graphs are citation networks, protein interaction graphs. That said, heterogeneous graphs might have several edge types (relations)
In KGs, we usually don't have such node type constraints, and any node can be connected with any other node

Similarity between heterogeneous graphs and KGs: both might have several edge types

Differences: node type structure in heterogeneous graphs is different from KGs 

\textit{(Input from Michael)}

\textit{Heterogeneous Graph:}
%https://www.emse.fr/~zimmermann/KGBook/Multifile/data-graphs/
A heterogeneous graph [Hussein et al., 2018, Wang et al., 2019, Yang et al., 2020] (or heterogeneous information network [Sun et al., 2011, Sun and Han, 2012]) is a directed graph where \textbf{each node and edge is assigned one type}. Heterogeneous graphs are thus akin to directed edge-labelled graphs – with edge labels corresponding to edge types – but where the type of node forms part of the graph model itself, rather than being expressed with a relation (as seen in Figure 2.2). An edge is called homogeneous if it is between two nodes of the same type (e.g., borders in Figure 2.2); otherwise it is called heterogeneous (e.g., capital in Figure 2.2). Heterogeneous graphs allow for partitioning nodes according to their type, for example, for the purposes of machine learning tasks [Hussein et al., 2018, Wang et al., 2019, Yang et al., 2020]. Conversely, such graphs typically only support a many-to-one relation between nodes and types, which is not the case for directed edge-labelled graphs 
\begin{figure}
    \centering
    \includegraphics{img/hetgraph.jpg}
    \caption{Comparing directed edge-labelled graphs and heterogeneous graphs}
    \label{fig:hetgraph}
\end{figure}
\textit{Knowledge Graph}

\subsection{Extrapolation vs. Interpolation}
\textit{Temporal Knowledge Graph Completion}: Given a Temporal Knowledge Graph \G with quadruples $(s,r,o,t)$ and $t \in T$, with $T = \{ 1 \ldots n \}, n \in \mathbb{N}^+$, \textit{TKG Completion} is the task of predicting missing information for known timesteps $t^k \leq n$ . 
This is usually done by link prediction, that is, predicting missing relations, or object or subject entities for queries $(s,?,o,t^k)$  $(s,r,?,t^k)$ or $(?,r,o,t^k)$.  \\

\textit{Temporal Knowledge Graph Forecasting}, also referred to as \textit{Temporal Knowledge Graph Extrapolation}: Given a Temporal Knowledge Graph \G with quadruples $(s,r,o,t)$ and $t \in T$, with $T = \{ 1 \ldots n \}, n \in \mathbb{N}^+$, \textit{TKG Forecasting} is the task of predicting quadruples for future timesteps $\tp$ with $\tp > n$ and $\tp \in \mathbb{N}^+$. 
In this work we focus on entity forecasting, that is, predicting object or subject entities for queries $(s,r,?,\tp)$ or $(?,r,o,\tp)$.  \\

Akin to (static) KG completion, TKG completion and forecasting are approached as a ranking task \cite{han2022TKG}. For a given query, e.g. \qt, methods rank all entities in $E$ using a scoring function, assigning plausibility scores to each quadruple. 



==> chapters/preliminaries/03_RelatedWork.tex <==
\subsection{{TKG Forecasting}}\label{sec:relwork_forecasting}
(\textit{Text in this section copied from \cite{gastinger2024baselines}})
\paragraph{Deep Graph Networks (DGNs)} Several models in this category leverage message-passing architectures \cite{scarselli2009,micheli2009} along with sequential approaches to integrate structural and sequential information for TKG forecasting. RE-Net adopts an autoregressive architecture, learning temporal dependencies from a sequence of graphs \cite{Jin2020renet}. RE-GCN combines a convolutional deep graph network with a sequential neural network and introduces a static graph constraint to consider additional information like entity types \cite{Li2021regcn}.
xERTE employs temporal relational attention mechanisms to extract query-relevant subgraphs \cite{Han2021xerte}. TANGO utilizes neural ordinary differential equations and DGNs to model temporal sequences and capture structural information \cite{Han2021tango}.
CEN integrates a convolutional neural network capable of handling evolutional patterns in an online setting, adapting to changes over time \cite{Li2022cen}. 
At last, RETIA generates twin hyperrelation subgraphs and aggregates adjacent entities and relations using a graph convolutional network \cite{Liu2023retia}.

\paragraph{Reinforcement Learning (RL)} Methods in this category combine reinforcement learning with temporal reasoning for TKG forecasting. CluSTeR employs a two-step process, utilizing a RL agent to induce clue paths and a DGN for temporal reasoning \cite{Li2020cluster}. Also, TimeTraveler leverages RL based on temporal paths, using dynamic embeddings of the queries, the path history, and the candidate actions to sample actions, and a time-shaped reward \cite{Sun21TimeTraveler}.

\paragraph{Rule-based} Rule-based approaches focus on learning temporal logic rules. TLogic learns these rules via temporal random walks, applying them to events prior to a query \cite{Liu2021tlogic}. TRKG extends TLogic by introducing new rule types, including acyclic rules and rules with relaxed time constraints \cite{Kiran2023TRKG}. ALRE-IR combines embedding-based and logical rule-based methods, capturing deep causal logic by learning rule embedding \cite{Mei2022alreir}. LogE-Net combines logical rules with RE-GCN, using them in a preprocessing step for assisting reasoning \cite{Liu2023logenet}. At last, TECHS incorporates a temporal graph encoder %utilizing a temporal encoding and heterogeneous attention, 
and a logical decoder for differentiable rule learning and reasoning \cite{Lin2023TECHS}. 

\paragraph{Others} There are additional approaches with mixed contributions that cannot be immediately placed in the above categories. CyGNet predicts future facts based on historical appearances, employing a "copy mode" and "generation mode" \cite{Zhu2021cygnet}. TiRGN employs a local encoder for evolutionary representations in adjacent timestamps %and periodicity in forecasting   
and a global encoder to collect repeated facts \cite{Li2022TiRGN}. 
CENET distinguishes historical and non-historical dependencies through contrastive learning and a mask-based inference process \cite{Xu2023CENET}.
Finally, L2TKG introduces a latent relation learning method, utilizing a structural encoder and latent relation learning module to mine and exploit intra- and inter-time latent relations \cite{Zhang2023L2TKG}. 

\textit{Comment Julia: I would suggest to start with the following models:}
\begin{itemize}
    \item TLogic (representative of rule-based category, relatively good results see Table~\ref{table:results}, code is ok and faster than others)
    \item RE-GCN (representative of DGN category, relatively good results see Table~\ref{table:results})
    \item TiRGN (representative of Others category, results are among the best for most datasets see Table~\ref{table:results}). However, I do not yet know their code.
    \item If we also want a representative from the RL category: Timetraveler (relatively good results). However, the code is a bit messy as far as I remember.
\end{itemize}



\subsection{{TKG Completion (Interpolation setting)}}
Two examples in this area of research are TeMP \cite{wu2020temp} and TNT Complex \cite{lacroix2019tensor} .
TeMP combine graph neural networks, temporal dynamics models, data imputation and frequency-based gating techniques to solve the TKG Completion task. 
TNT Complex extends the ComplEx model for TKG Completion by augmenting it with timestamp embeddings. Based on the assumption that timestamp representations evolve slowly over time, the paper introduces this prior as a regularizer. Further, they add a non-temporal component to the model to deal with static facts in knowledge bases. 
Note: The paper itself might not be relevant for us, but they introduce \textbf{another version of WIKI which might be worth checking} @Andy. % the wiki dataset seems a bit complicated though in that it only should be used for predictions in one direction (s,r,?,t) and not (?,r,o,t) 

\textit{Comment Julia: I would suggest to not include works from the TKG Completion category in TGB 2.0, because it is a different task than forecasting. I just added them for reference.}

\subsection{THG}
TODO

==> chapters/preliminaries/04_Datasets.tex <==
\subsection{TKG: state-of-the-art}
(\textit{Text in this section copied from \cite{gastinger2023eval}})

Researchers in the domain of TKG Forecasting use the following datasets:
Three instances of ICEWS \cite{Boschee2015}: ICEWS05-15 \cite{GarciaDuran2018ICEWS14}, ICEWS14 \cite{GarciaDuran2018ICEWS14}, and ICEWS18 \cite{Jin2019oldrenet}, where the numbers mark the respective years; further, YAGO \cite{Mahdisoltani2015YAGO} and WIKI \cite{Leblay2018WIKI}, preprocessed according to \cite{Jin2019oldrenet}, as well as GDELT \cite{Leetaru2013GDELT}. %The supplementary material contains dataset statistics.
Table~\ref{table:datasets} shows dataset statistics for dataset version (a), as reported by \cite{Li2021regcn}.

The models described in Section~\ref{sec:relwork_forecasting} report results on different versions of the same dataset. For instance, three versions exist for ICEWS14. 

\begin{table}[hbt!]
\caption{Dataset Statistics for dataset version (a), as reported by \cite{Li2021regcn} and as proposed by \cite{gastinger2023eval} to be used in unified evaluation protocol.}
\centering
\begin{tabular}{lrrrrrr}
%{p{  1.5cm} p{   1.0cm} p{   0.9cm} p{   1.8cm} p{   2.1cm} p{   1.9cm}p{   1.9cm}} %{lrrrrrr}
\toprule
Dataset &  $\#$Nodes &  $\#$Rels& $\#$Train & $\#$Valid & $\#$Test & Time Interval\\
\midrule
ICEWS14 &  $7128$ 	&  $230$ 	& $74845$	& $8514$	& $7371$	& 24 hours\\
ICEWS18 &  $23033$ 	&  $256$ 	& $373018$ 	& $45995$ 	& $49545$ 	& 24 hours \\
ICEWS0515 &  $10094$ 	&  $251$ 	& $368868$	& $46302$	& $46159$	& 24 hours\\ %4017 timestamps
GDELT &  	$7691$ 	&  $240$ 	& $1734399$& $238765$	& $305241$	& 15 minutes\\
YAGO &  	$10623$ 	&  $10$ 	& $161540$	& $19523$	& $20026$	& 1 year\\
WIKI &  	$12554$ 	&  $24$ 	& $539286$	& $67538$	& $63110$	& 1 year\\
%TODO: talk also about ICEWS2021 and ACLED from zifeng paper
\bottomrule
\end{tabular}
\label{table:datasets}
\end{table}

\subsection{TKG: added datasets}
\textcolor{red}{todo add links}
\begin{itemize}
    \item WIKI
    \item POLECAT
    \item ICEWS
\end{itemize}



\begin{table*}[t] %\vspace{-12pt}
\caption{Dataset Statistics. Dataset names are colored based on their scale as \textcolor[HTML]{e7298a}{small}, \textcolor{blue}{medium}, and \textcolor[HTML]{1b9e77}{large}.
% \textit{$*$}: The time granularity of the datasets are noted in parentheses with \textit{U-ts}, \textit{D}, and \textit{Y} denoting UNIX timestamps, day, and year, respectively.
\textit{$^\P$}: Edges can be \textit{\textbf{W}eighted}, \textit{\textbf{Di}rected}, or  \textit{\textbf{A}ttributed}.} %\vspace{-5pt}
\label{tab:stats-summarized}
  \resizebox{\textwidth}{!}{%
  \begin{tabu}{l l | l l l l l l l l}
  \toprule
  \toprule
   & Dataset & Domain & \# Nodes & \# Edges &  \# Steps  & Surprise & # E.Types & # Node.Types & Edge Properties\textit{$^\P$} \\ % & \# Edge Features  \\
  %& Time Granularity
  \midrule
  \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{TKG}}} &
  \textcolor[HTML]{e7298a}{\polecat} & political & xxx & xxx & xxx & xxx & xxx & \xmark & W: \xmark, Di: \cmark, A: \cmark\\
   & \textcolor{blue}{\icews} & political & xxx & xxx & xxx & xxx & xxx & \xmark & W: \cmark, Di: \cmark, A: \xmark\\
   & \textcolor[HTML]{1b9e77}{\wikidata}  & knowledge & xxx & xxx & xxx & xxx & xxx & \xmark & W: \cmark, Di: \cmark, A: \xmark\\
   % & \textcolor[HTML]{1b9e77}{\reddit}                          & social & 994,790 & 44,314,507 & 30,998,030 & 0.823 & W: \cmark, Di: \cmark, A: \cmark\\
   % & \textcolor[HTML]{1b9e77}{\sky}                            & traffic & 18143 & 67,169,570 & 1,385 & 0.024 & W: \xmark, Di: \cmark, A: \cmark \\ % & 172 \\
  
  \midrule
  \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{THG}}} & 
  \textcolor[HTML]{e7298a}{\github}     & software & 133,066 & 281,295 & xxx & xxx & 18 & 6 & W: \cmark, Di: \cmark, A: \xmark\\ % & 4 \\
  % & \textcolor{blue}{}                              & interact.  & \changed{1,505} & 17,858,395 & 133,758 & 0.005 & W: \cmark, Di: \cmark, A: \xmark\\
  & \textcolor[HTML]{1b9e77}{\myket}   & interact. & xxx & xxx & xxx & xxx & 2 & 2 & W: \cmark, Di: \cmark, \changed{A: \xmark}\\   %A: \cmark
  \bottomrule
  \bottomrule
  \end{tabu}
  }
\end{table*}



\subsection{THG}






==> chapters/preliminaries/05_EvaluationProtocol.tex <==
\subsection{TKG}
(\textit{Text in this section copied from \cite{gastinger2023eval}})

\subsubsection{Single-step vs. Multi-step}
Methods for Forecasting operate within two distinct prediction settings, single-step and multi-step prediction.
Single-step (or one-step) prediction means that the model always forecasts the next timestep \cite{brownlee2018singlestep}. The ground truth facts 
are then fed before predicting the subsequent timestep.  
Multi-step prediction means that the model forecasts more than one future time step \cite{brownlee2018singlestep}. More specifically, the model predicts all timesteps from the test set, without seeing any ground truth information in between. 
As described by \cite{brownlee2018singlestep}, multi-step prediction is more challenging, as the model can only leverage information from its own forecasts, and uncertainty accumulates with an increasing number of forecasted timesteps.

\textbf{We report results in single-step setting.}

\subsubsection{Negative Sampling}
Currently, the methods described in \ref{sec:relwork_forecasting} do not do Negative Sampling, but compute results on the full node set, i.e. 1-vs-all strategy.

\subsubsection{Evaluation Metrics: Filter Settings}
Commonly, in link prediction evaluations, results are reported on the following metrics: the Mean Reciprocal Rank (MRR), computing the average of the reciprocals of the ranks of the first relevant item in a list of results, as well as the Hits at $k$ (H@k), the proportion of queries for which at least one relevant item is among the top $k$ ranked results. 

\textit{Time-aware filter}: \cite{Han2020ghnn} note that the static filter setting is inappropriate for temporal link prediction because it filters out all triples that have ever appeared from the list of corrupted triples, ignoring the time validity of facts. As a consequence, it does not consider predictions of such triples as erroneous. 
For example, if there is a test query (Barack Obama, visit, India, 2015-01-25) and if the train set contains (Barack Obama, visit, Germany, 2013-01-18), the triple (Barack Obama, visit, Germany) is filtered out for the test query according to the static filter setting, even though it is not true for 2015-01-25 \cite{Han2021xerte}. 
For this reason, numerous works \cite{Han2021xerte,  Liu2021tlogic, Han2021tango, Sun21TimeTraveler, Li2022cen, Li2020cluster, gastinger2023eval, gastinger2024baselines} apply the \textit{time-aware filter} setting which only filters out quadruples with the same timestamp as the test query. In the above example, (Barack Obama, visit, Germany, $t$) would only be filtered out for the given test query, if it had the timestamp $t=$~2015-01-25, and otherwise stay in the list of corrupted triples.

\textbf{We report the time-aware filtered MRR.}


\subsection{THG}
is it a different protocol?

==> chapters/preliminaries/06_CurrentResults.tex <==
\subsection{TKG}
(\textit{Text in this section copied from \cite{gastinger2024baselines}}. )
 
For Reference - to potentially identify which models to include


We report results for 11 among the 17 methods described in Section~\ref{sec:relwork_forecasting}, plus the recurrency baseline \cite{gastinger2024baselines}. 
Two of these 17 methods run only in multi-step setting. %We include results in the multi-step analysis in Appendix~\ref{section:appmulti}.
Further, for four methods we find discrepancies in the evaluation protocol and thus exclude them from our comparisons\footnote{CENET, RETIA, and CluSTER do not report results in time-aware filter setting. ALRE-IR does not report results on WIKI, YAGO, and GDELT, and uses different dataset versions for ICEWS14 and ICEWS18.}.

Unless otherwise stated, we report the results for these 11 methods based on the evaluation protocol by \cite{gastinger2023eval}. For TiRGN, we report the results of the original paper and do a sanity check of the released code. We do the same for L2TKG, LogE-Net, and TECHS, but we cannot do a sanity check as the authors have not released their code. 
 
\setlength{\tabcolsep}{5pt}
\begin{table*}
\caption{Experimental results for single-step prediction. An entry ${\dagger}$ means authors have not released their code, and thus we could not reproduce their results. 
An entry - means that the related work does not report results on this dataset. An entry "d.d.v" means, that the related work reports results on a different dataset version.}
\label{table:results}
\small
% \scriptsize
\centering
\begin{tabular}{l|rr|rr|rr|rr|rr}
\toprule
& \multicolumn{2}{c|}{GDELT} & \multicolumn{2}{c|}{YAGO} & \multicolumn{2}{c|}{WIKI} & \multicolumn{2}{c|}{ICEWS14} & \multicolumn{2}{c}{ICEWS18} \\
\midrule
		                  & MRR  & H@10 & MRR  & H@10 & MRR  & H@10 & MRR & H@10 & MRR & H@10  \\
\midrule
L2TKG$^{\dagger}$     & 20.5          & 35.8          & -             & -             & -             & -             & \textbf{47.4} & \textbf{71.1} & \ul{{33.4}} & \textbf{55.0} \\
LogE-Net$^{\dagger}$  & -             & -             & -             & -             & -             & -             & 43.7          & 63.7          & 32.7                & 53.0          \\
TECHS$^{\dagger}$     & -             & -             & 89.2          & 92.4          & 76.0          & 82.4          & d.d.v         & d.d.v.        & 30.9                & 49.8          \\
TiRGN                  & \ul{21.7}          & \ul{37.6}          & 88.0          & \ul{92.9}     & \ul{81.7}     & \textbf{87.1} & \ul{44.0}     & \ul{63.8}     & \textbf{33.7}       & \ul{54.2}    \\
TRKG                   & 21.5          & 37.3          & 71.5          & 79.2          & 73.4          & 76.2          & 27.3          & 50.8          & 16.7                & 35.4          \\
RE-GCN                 & 19.8          & 33.9          & 82.2          & 88.5          & 78.7          & 84.7          & 42.1          & 62.7          & 32.6                & 52.6          \\
xERTE                  & 18.9          & 32.0          & 87.3          & {91.2}        & 74.5          & {80.1}        & 40.9          & 57.1          & 29.2                & 46.3          \\
TLogic                 & 19.8          & 35.6          & 76.5          & 79.2          & \textbf{82.3} & 87.0          & 42.5          & 60.3          & 29.6                & 48.1          \\
TANGO                  & 19.2          & 32.8          & 62.4          & 67.8          & 50.1          & 52.8          & 36.8          & 55.1          & 28.4                & 46.3          \\
Timetraveler & 20.2          & 31.2          & 87.7          & 91.2          & 78.7          & 83.1          & 40.8          & 57.6          & 29.1                & 43.9          \\
CEN                    & 20.4          & 35.0          & 82.7          & 89.4          & 79.3          & 84.9          & 41.8          & 60.9          & 31.5                & 50.7          \\
Baseline ($\psi_\Delta\xi$)      & \textbf{24.5} & \textbf{39.8} & \textbf{90.9} & \textbf{93.0} & 81.5          & \textbf{87.1} & 37.2          & 51.8          & 28.7                & 43.7          \\ %updated 22.12.
\bottomrule
  \end{tabular}
\end{table*}



==> chapters/preliminaries/copy_Datasets_copy_5_30.tex <==
\textbf{Dataset Categorization}
\name features \todo{six} temporal multi-relational graph datasets, \todo{six} of which have been collected and curated for this work. 

When examining runtime and memory consumption across methods, we observe an increasing difficulty from \smallpedia to \polecat to \icews and \wikidata, when it comes to runtimes and memory requirements. The same is true for the THG datasets. This cannot be solely attributed to a single metric but rather hinges on factors such as the number of nodes, timesteps, and quadruples. Thus, based on practical consideration in benchmarking efforts, we categorize the datasets into the labels \smalld{small}, \mediumd{medium}, and \larged{large}.

We split all datasets chronologically into the training, validation, and test sets, respectively containing $70\%$, $15\%$, and $15\%$ of all edges, in line with similar studies such as \todo{cite [48, 35, 45, 20, 40, 25]} and ensure that edges for a timestep can only be in either train or validation or test set. \jg{should we put in the appendix the number of train/valid/test timesteps? its not obvious because of splitting based on number of triples and then ensuring that the same timestep is not in train and valid or valid and test set. }
We present the dataset licenses and download links in Appendix\ref{app:license}, and the datasets will be permanently maintained via Digital Research Alliance of Canada funded by the Government of Canada.

Table~\ref{tab:datasetstats} shows characteristics of all datasets, such as the number of Quadruples and Nodes.
In addition, we report the Degree of Inductive Test nodes, i.e. nodes in the test set that have not been seen in the train set. Further, we the fraction of test temporal triples $(s,r,o,\tp)$ for which there exists a $k<\tp$ such that $(s,r,o,k) \in G$, the \textit{Recurrency Degree (Rec)}. We also compute the fraction of temporal triples $(s,r,o,\tp)$ for which it holds that $(s,r,o,\tp-1) \in G$, the \textit{direct} recurrency degree \textit{(DRec)} \cite{gastinger2024baselines}.
To quantify whether a dataset is more event-based, or fact-based, in addition to the existing measures, we compute a novel value termed \textit{Consecutiveness Value} (Con) to further characterize the temporal nature of datasets. To compute the Con, for each triple in the dataset, we identify the maximum number of consecutive timesteps during which the triple holds true and average this across all triples in the dataset. 
Further, Figures~\ref{fig:edges_time_tkg} and ~\ref{fig:edges_time_thg} show the number of edges per timestep. %The figure highlights the diversity in datasets.
For the TKG datasets, we illustrate the distribution of the ten most prominent relations in Figure~~\ref{fig:pie}.

From Table~\ref{tab:datasetstats} and Figures~\ref{fig:edges_time_tkg},~\ref{fig:edges_time_thg}, and~\ref{fig:pie} several key observations emerge:

Firstly, there is a {notable variation in dataset sizes}, encompassing differences in the number of nodes, edges, and time steps. 

Moreover, distinct properties in terms of fact duration and repetition are evident across datasets: Notably, the high Consecutiveness degree for \smallpedia and \wikidata exhibit a prevalence of long-lasting facts, contrasting with \icews and \polecat, as well as the THG datasets, which are more event-centric. 
Additionally, variations in the recurrence of facts are apparent, with datasets \smallpedia and \wikidata showing a higher Recurrency Degree as compared to others. 
Notably, the direct recurrence degree highlights disparities between THG and TKG datasets, where the time granularity of "seconds" of THG leads to a direct recurrence degree of 0, implying no repetition of facts across subsequent time steps. 

Furthermore, Figures~\ref{fig:edges_time_tkg} and~\ref{fig:edges_time_thg} underscore distinctions between datasets, particularly in terms of time granularity and trend patterns. TKG datasets demonstrate a coarser time granularity leading to a significantly higher edge count per timestep compared to THG datasets. 

While most datasets exhibit fluctuations in the number of edges around a constant level, \wikidata stands out with a significant upward trend in the number of edges over the years, indicating a surge in events, particularly in recent years.

In addition, noteworthy deviations in timesteps are apparent. TKG datasets display anomalous timesteps characterized by minimal edge numbers, particularly evident during the Covid pandemic for \icews. Conversely for the THG datasets the occurrence of zero-edge timesteps is not indicative of outliers; rather, it reflects the continuous nature of the data, where not every second entails an event occurrence. Conversely, THG datasets exhibit instances of exceptionally high edge counts per timestep, such as in the case of \forum with up to 120 edges per timestep.

Figure~~\ref{fig:pie} highlights that \smallpedia is dominated by \todo{TODO describe what we see from the pie charts.}

% What we see from table and figures:
% \begin{itemize}
%     \item dataset diversity: 
%     \begin{itemize}
%         \item various different sizes (in terms of number of nodes, edges, timesteps)
%         \item different properties in times of fact repetition: e.g., \smallpedia and \wikidata have more longlasting facts (e.g. people being married with each other for a longer time), wheres \icewas and \polecat, as well as the THG datasets are more event based (see consecutiveness degree).
%         \item some datasets have a high amount of recurring facts (see Recurrency Degree), e.g., \smallpedia and \wikidata, whereas others don't.
%         \item from the direct recurrency degree we see the difference between THG and TKG: because of the continuous time setting and the nature of the datasets, the THG datasets have direct recurrency degree of 0: if a fact happens at one timestep, it does not reoccur at the subsequent timestep. For example, if a user posts in a forum, they do not have done a post in the same forum a second ago.
%     \end{itemize}
%     \item The figures also highlight the differences in datasets:
%     \begin{itemize}
%         \item For the TKG datasets, we have a much coarser time granularity, and thus significantly more edges per timestamp as compared to the THG datasets
%         \item Trend: Wheres for most datasets the number of edges fluctuate around a constant level, for \wikidata we see a very significant upward trend in number of edges over the years, with most events happening in the last bin.
%         \item Outlier timesteps: For TKG with (close to) zero edges, e.g. for \icews (during Covid). for THG we have timesteps with significantly more number of edges, reaching e.g. up to 120 for \forum. Further, for THG we have a lot of timesteps with zero edges, due to the continuous property of the dataset
%     \end{itemize} 
% \end{itemize}
% \todo{describe what the stats as well as the figure tell us. dataset diversity, types (fact based event based), periodicity, evolvement over time, outliers, size.}
% \todo{Explain all stats in the table. @julia in appendix or here if space permits. Particularly explain by DRec is 0 for all thgl datasets due to them not having recurring edges in the immediate previous step (no duration based relation types).}

Next, we described the details of each dataset. 

\subsection{Temporal Knowledge Graphs} \todo{to be written by Andy}

\smallpedia. This dataset is constructed from the \href{https://www.wikidata.org/wiki/Wikidata:Database_download}{WikiData Database} where it contains the relations extracted from \href{https://en.wikipedia.org/wiki/Main_Page}{Wikipedia} pages. The head and tails are entities. The relations are properties descrbing entities. \smallpedia is extracted from wikidata pages where the entities ID is less or equal than 1 million. The temporal relations are extracted from properties with qualifiers that are either point in time or has a start or end date. 


\polecat. This dataset is \href{https://dataverse.harvard.edu/dataset.xhtml?persistentId=doi:10.7910/DVN/AJGVIT}{data source link}


\icews. This dataset \href{https://dataverse.harvard.edu/dataset.xhtml?persistentId=doi:10.7910/DVN/28075}{data source link}

\wikidata. This dataset \href{https://www.wikidata.org/wiki/Wikidata:Database_download}{WikiData Json Data Dump} \todo{ANDY: talk about the static info for wikidata and smallpedia}

\subsection{Temporal Heterogeneous Graphs} \todo{to be written by Andy}
\paragraph{thgl-software} Github dataset is collected from \href{https://www.gharchive.org/}{GH Arxiv}. We filter to keep only nodes with at least 10 edges in a month. The dataset is for 2024-01.

\paragraph{thgl-github} Github dataset is collected from \href{https://www.gharchive.org/}{GH Arxiv}. We retain user, pull request, issue and repository nodes. Then nodes with two or less edges are removed. 

\paragraph{thgl-forum} The data source is \href{https://surfdrive.surf.nl/files/index.php/s/M09RDerAMZrQy8q#editor}{here}~\cite{nadiri2022large}.

\paragraph{thgl-myket} The full set of Myket dataset similar to \href{https://github.com/erfanloghmani/myket-android-application-market-dataset}{the small version}~\cite{loghmani2023effect}.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{img/num_edges_discretized_20_tkgl-polecat2.pdf}
%     \caption{Placeholder for dataset figures. Mean Number of Triples per timestep for all datasets. \todo{Include figures for all 8 datasets}}
%     \label{fig:triples_ts}
% \end{figure}

\begin{figure*}[!t]
\begin{minipage}{.48\textwidth}
	\centering
\small{(a) \polecat}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_tkgl-polecat2.pdf}\\
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
\small{(b) \icews}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_tkgl-icews2.pdf}\\
\end{minipage}
\begin{minipage}{.48\textwidth}
	\centering
\small{(c) \smallpedia}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_tkgl-smallpedia2.pdf}\\
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
\small{(d) \wikidata}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_tkgl-wikidata2.pdf} \\
\end{minipage}
\caption{Dataset Edges over time for TKG.} 
	\label{fig:edges_time_tkg}
\end{figure*}

\begin{figure*}[!t]
\begin{minipage}{.48\textwidth}
	\centering
\small{(e) \software}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_thgl-software2.pdf} \\
	%\subcaption{\label{fig:b900}Multistep ICEWS18.}
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
\small{(f) \forum}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_thgl-forum2.pdf}  \\
%	\subcaption{Budget 30 minutes.} 
\end{minipage}
\begin{minipage}{.48\textwidth}
	\centering
\small{(e) \myket}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_thgl-myket2.pdf} \\
	%\subcaption{\label{fig:b900}Multistep ICEWS18.}
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
\small{(f) \github}
	\includegraphics[width=\textwidth]{img/num_edges_discretized_20_thgl-github2.pdf}  \\
%	\subcaption{Budget 30 minutes.} 
\end{minipage}
\caption{Dataset Edges over time for THG. } 
	\label{fig:edges_time_thg}
\end{figure*}



\begin{figure*}[!t]
\begin{minipage}{.48\textwidth}
	\centering
\small{(a) \polecat}
	\includegraphics[width=\textwidth]{img/rel_pie_tkgl-polecat.pdf} \\
	%\subcaption{\label{fig:b900}Multistep ICEWS18.}
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
 \small{(b) \smallpedia}
	\includegraphics[width=\textwidth]{img/rel_pie_tkgl-smallpedia.pdf} \\
	%\subcaption{\label{fig:b900}Multistep ICEWS18.}
\end{minipage}

\begin{minipage}{.48\textwidth}
	\centering
\small{(c) \icews}
	\includegraphics[width=\textwidth]{img/rel_pie_tkgl-icews.pdf}  \\
%	\subcaption{Budget 30 minutes.} 
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
	\centering
\small{(d) \wikidata}
	\includegraphics[width=\textwidth]{img/rel_pie_tkgl-wikidata.pdf}  \\
%	\subcaption{Budget 30 minutes.} 
\end{minipage}
\caption{Pie charts } 
	\label{fig:pie}
\end{figure*}



\todo{Figure about the distribution of relation types per dataset, something like a fancy pie-chart}

\begin{table}[]
\caption{Dataset Statistics. Among common dataset statistics, we report the factor of Inductive Test nodes (Induct. Test Nodes), the Direct Recurrency Degree (DRec), the Recurrency Degree (Rec), the Consecutiveness Value (Con), as well as the mean number of edges and nodes per timestep (Mean Edges/Ts. and Mean Nodes/Ts.)}
\label{tab:datasetstats}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|rrrr|rrrr}
\toprule
                           & \multicolumn{4}{c|}{Temporal Knowledge Graphs}                                                    & \multicolumn{4}{c}{Temporal Heterogenous Graphs}                                                \\
                           \midrule
Dataset             & \smalld{\smallpedia}  & \mediumd{\polecat} & \larged{\icews} & \larged{\wikidata} & \smalld{\software} & \mediumd{\forum} & \larged{\github} & \larged{\myket}  \\
\midrule
Domain                  &  knowledge    & political               & political             & knowledge                  & software               & social.             & software  & interac.  \\
\# Quadruples           & 550,376       & 1,779,610           & 15,513,446        & 9,856,203                              & 1,489,806            & 23,757,707        & 17,499,577 & 53,632,788    \\
\# Nodes                & 47,433        & 150,931             & 87,856            & 1,226,440                               & 681,927            & 152,816            & 5,856,765 & 1,530,835 \\
\# Edge Types           &  283          & 16                  & 391               & 596                                        & 14                 & 2               & xxx  & 2  \\
\# Node Types           & \xmark        & \xmark   & \xmark & \xmark                                                        & 4                     & 2                & 4            & 2               \\
\# Timesteps            & 125           & 1,826               & 10,224            & 2,025                                       & 689,549            & 2,558,457          & xxx & 14,828,090       \\
Granularity             & year          & day                     & day                   & year                               & second                 & second           & xxx     & second   \\            
\midrule[0.5pt]
Induct. Test Nodes      & 0.26          & 0.12                    & 0.05                  & 0.34                                 & 0.13                  & 0.02                 & xxx   & 0.01         \\
DRec                    & 0.71          & 0.07                    & 0.11                  & 0.61                                 & 0.00                   & 0.00                & xxx   & 0.00          \\
Rec                     &  0.72         & 0.43                    & 0.63                  & 0.61                               & 0.10                  & 0.63                   &  xxx  & 0.37           \\
Con                     & 5.82          & 1.07                    & 1.14                  & 5.05                                 & 1.00                  & 1.00                 & xxx   & 1.00     \\
Mean Edges/Ts.          & 4,403.01      & 974.59                  & 1,516.91              & 4,867.26                       & 0.56                   & 8.87                      & xxx   & 3.15        \\
Mean Nodes/Ts.          & 5,289.16      & 550.60                  & 1,008.65              & 5,772.16                       & 0.86                   & 12.96                     & xxxx  & 6.24        \\

 \bottomrule
\end{tabular}
}
\end{table}




% \begin{table*}[t] %\vspace{-12pt}
% \caption{Dataset Statistics. Dataset names are colored based on their scale as \smalld{small}, \mediumd{medium}, and \larged{large} \textcolor{blue}{TODO these numbers are including inverses, divide by two for num edges}.
% % \textit{$*$}: The time granularity of the datasets are noted in parentheses with \textit{U-ts}, \textit{D}, and \textit{Y} denoting UNIX timestamps, day, and year, respectively.
% } %\vspace{-5pt}
% \label{tab:stats-summarized}
%  \resizebox{\textwidth}{!}{%
%   \begin{tabu}{l l | l r r r r r r r}
%   \toprule
%   \toprule
%    & Dataset & Domain & \# Nodes & \# Edges &  \# Steps  & Surprise & \# E.Types & \# N.Types & Granularity \\ % & \# Edge Features  \\
%   %& Time Granularity
%   \midrule
%   \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{TKG}}} &
%   \smalld{\polecat} & political & 150,931 & 3,559,220 & 1,826 & xxx & 16 & \xmark & day\\
%    & \mediumd{\icews} & political & 87,856 & 31,026,892 & 10,224 & xxx & 391 & \xmark & day\\
%    & \larged{\wikidata}  & knowledge  &1,226,440 & 19,712,406 &2,025 & xxx & 596 & \xmark & year\\
%    % & \larged{\reddit}                          & social & 994,790 & 44,314,507 & 30,998,030 & 0.823 & W: \cmark, Di: \cmark, A: \cmark\\
%    % & \larged{\sky}                            & traffic & 18143 & 67,169,570 & 1,385 & 0.024 & W: \xmark, Di: \cmark, A: \cmark \\ % & 172 \\
  
%   \midrule
%   \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{THG}}} & 
%   \smalld{\github}     & software & 133,066 & 281,295 & xxx & xxx & 18 & 6 & second \\ % & 4 \\
%   & \mediumd{\forum} & social. & xxx & xxx & xxx & xxx & 2 & 2 & second \\
%   % & \mediumd{}                              & interact.  & \changed{1,505} & 17,858,395 & 133,758 & 0.005 & W: \cmark, Di: \cmark, A: \xmark\\
%   & \larged{\myket}   & interact. & 1,530,835 & 107,265,576 & 14,828,090 & xxx & 2 & 2 & second \\   %A: \cmark
%   \bottomrule
%   \bottomrule
%   \end{tabu}
% }
% \end{table*}


% \begin{table*}[t] %\vspace{-12pt}
% \caption{Dataset Statistics. Dataset names are colored based on their scale as \smalld{small}, \mediumd{medium}, and \larged{large}.
% % \textit{$*$}: The time granularity of the datasets are noted in parentheses with \textit{U-ts}, \textit{D}, and \textit{Y} denoting UNIX timestamps, day, and year, respectively.
% \textit{$^\P$}: Edges can be \textit{\textbf{W}eighted}, \textit{\textbf{Di}rected}, or  \textit{\textbf{A}ttributed}.} %\vspace{-5pt}
% \label{tab:stats-summarized}
%  \resizebox{\textwidth}{!}{%
%   \begin{tabu}{l l | l l l l l l l l}
%   \toprule
%   \toprule
%    & Dataset & Domain & \# Nodes & \# Edges &  \# Steps  & Surprise & \# E.Types & \# N.Types & Edge Properties\textit{$^\P$} \\ % & \# Edge Features  \\
%   %& Time Granularity
%   \midrule
%   \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{TKG}}} &
%   \smalld{\polecat} & political & xxx & xxx & xxx & xxx & xxx & \xmark & W: \xmark, Di: \cmark, A: \cmark\\
%    & \mediumd{\icews} & political & xxx & xxx & xxx & xxx & xxx & \xmark & W: \cmark, Di: \cmark, A: \xmark\\
%    & \larged{\wikidata}  & knowledge & xxx & xxx & xxx & xxx & xxx & \xmark & W: \cmark, Di: \cmark, A: \xmark\\
%    % & \larged{\reddit}                          & social & 994,790 & 44,314,507 & 30,998,030 & 0.823 & W: \cmark, Di: \cmark, A: \cmark\\
%    % & \larged{\sky}                            & traffic & 18143 & 67,169,570 & 1,385 & 0.024 & W: \xmark, Di: \cmark, A: \cmark \\ % & 172 \\
  
%   \midrule
%   \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{THG}}} & 
%   \smalld{\github}     & software & 133,066 & 281,295 & xxx & xxx & 18 & 6 & W: \cmark, Di: \cmark, A: \xmark\\ % & 4 \\
%   & \mediumd{\forum} & social. & xxx & xxx & xxx & xxx & xxx & \xmark & W: \cmark, Di: \cmark, A: \xmark\\
%   % & \mediumd{}                              & interact.  & \changed{1,505} & 17,858,395 & 133,758 & 0.005 & W: \cmark, Di: \cmark, A: \xmark\\
%   & \larged{\myket}   & interact. & xxx & xxx & xxx & xxx & 2 & 2 & W: \cmark, Di: \cmark, \changed{A: \xmark}\\   %A: \cmark
%   \bottomrule
%   \bottomrule
%   \end{tabu}
% }
% \end{table*}



==> chapters/preliminaries/copy_related_work.tex <==
In the following, we describe recently proposed methods for future link prediction in multi-relational graphs, datasets used to evaluate these approaches, as well as related work on benchmarking. 
\subsection{Methods}\label{sec:relwork_methods}
For \textbf{TKG} Forecasting, multiple methods have been proposed in recent years. All but one (\cite{Han2020ghnn}) utilize a discrete time representation.
Some methods integrate message-passing architectures~\cite{scarselli2009,micheli2009}  with sequential techniques (~\cite{Jin2020renet,Li2021regcn,Han2021xerte,Han2021tango,Li2022cen,Liu2023retia}). Others (~\cite{Li2020cluster,Sun21TimeTraveler}) combine Reinforcement Learning with temporal reasoning to forecast future links. Additionally, certain methods (\cite{Liu2021tlogic, Kiran2023TRKG, Mei2022alreir, Liu2023logenet, Lin2023TECHS}) employ rule-based strategies to learn temporal logic rules, while others \cite{Zhu2021cygnet,Xu2023CENET,Zhang2023L2TKG} offer a blend of other methodologies.
%Further details are provided in Appendix~\ref{sec:relwork_tkg_forecasting}. In this work we undertake a comparative analysis, selecting at least one method from each of the aforementioned categories, facilitated by \name.

In the research field of \textbf{THG}, several methods have been developed, categorized into two main groups: those operating on discrete-time, processing sequences of discrete snapshots, and those operating on continuous time. Given the broader applicability of the continuous-time approach and the recent surge in proposed methods, within this framework we concentrate on approaches utilizing continuous time. The contributions in this context encompass a variety of techniques, including probabilistic modeling (\cite{ji2021dynamic, sajadmanesh2019continuous}), temporal extensions of message passing architectures (\cite{rossi2020temporal}), methods employing attention mechanism %\cite{li2020heterogeneous, luo2020dynamic}. 
\todo{what about \cite{li2023simplifying} STHN where does this go?}. 

We compare a selected subset of above methods in section~\ref{sec:results}. Further elaboration on these methods is available in Appendix~\ref{sec:relwork_thg_forecasting}.

\subsection{Multi-relational Temporal Graph Datasets}\label{sec:relwork_datasets}
\textbf{TKG: } For Temporal Knowledge Graph Forecasting, typically the following datasets are used: three instances of the Integrated Crisis Early Warning System (ICEWS) \cite{Boschee2015}: ICEWS05-15 \cite{GarciaDuran2018ICEWS14}, ICEWS14 \cite{GarciaDuran2018ICEWS14}, and ICEWS18 \cite{Jin2019oldrenet}, ICEWS21-zero and ICEWS22-zero~\cite{Ding2024zrllm}, where the numbers mark the respective years; further, YAGO \cite{Mahdisoltani2015YAGO} and WIKI \cite{Leblay2018WIKI}, preprocessed according to \cite{Jin2019oldrenet}, as well as GDELT \cite{Leetaru2013GDELT}. In addition, recently~\cite{Ding2024zrllm} introduced three newer datasets, ICEWS21-zero, ICEWS22-zero, two more recent instances of ICEWS\cite{Boschee2015} and ACLED-zero, curated from the Armed Conflict Location and Event Dataset~\cite{raleigh2010acled}.
It's worth noting that according to~\cite{gastinger2024baselines}, YAGO should primarily be used as a sanity check dataset rather than for measuring progress due to its limited potential for improvement. Additionally, the ICEWS datasets consist of subsets from specific years and available nodes, restricting the capability for long-range predictions. Similarly, the WIKI dataset covers only a subset of years and significantly fewer nodes compared to alternative versions. Consequently, current evaluation datasets for TKG forecasting methods typically feature a smaller scale in terms of nodes, relations, edges, and/or timesteps. This is also visible in Figure~ref{fig:dataoldnewtkg} which presents a comparative analysis of dataset statistics from prior research and those introduced by \name. Notably, the datasets introduced by \name demonstrate a significant leap in scale, surpassing prior datasets by an order of magnitude in terms of the number of nodes, edges, and/or timesteps.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/dataset_statstkg}
%     \caption{\ah{two figures here, one for TKG, one for THG, change styling.} Placeholder for dataset size olf vs new figure. \todo{TODO: add THG. TODO: add legend describing the num timesteps.}}
%     \label{fig:dataoldnewtkg}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth} % Adjust the width as needed
%         \includegraphics[width=\textwidth]{img/dataset_statstkg} % Image for TKG
%         \caption{Caption for TKG figure}
%         \label{fig:dataoldnewtkg}
%     \end{subfigure}
%     \hfill % This command adds horizontal space between subfigures
%     \begin{subfigure}[b]{0.45\textwidth} % Adjust the width as needed
%         \includegraphics[width=\textwidth]{img/dataset_statsthg.pdf} % Image for THG
%         \caption{Caption for THG figure}
%         \label{fig:dataoldnewthg}
%     \end{subfigure}
%     \caption{Placeholder for dataset size comparison.}
%     \label{fig:dataoldnew}
% \end{figure}



% \begin{figure*}[!t]
% \begin{minipage}{.48\textwidth}
% 	\centering
% 	\includegraphics[width=\textwidth]{img/dataset_statstkg.pdf}
%         \small{(a)} \\
% %\small{(a)}
% 	%\subcaption{\label{fig:b900}Multistep ICEWS18.}
% \end{minipage}
% \hfill
% \begin{minipage}{.48\textwidth}
% 	\centering
% 	\includegraphics[width=\textwidth]{img/dataset_statsthg.pdf}
%         \small{(b)}\\

% 	%\subcaption{Budget 30 minutes.}
% \end{minipage}

% \caption{Datasets used in related work (yellow) vs. datasets presented in \name for TKG (a), red and THG (b), green. The size of the circles indicates the number of timestamps. Most \name datasets are orders of magnitude larger as compared to existing datasets.}
% 	\label{fig:dataoldnewtkg}
% \end{figure*}



\textbf{THG: } \todo{Shortly describe and reference existing datasets and differences to our datasets}.
%
\subsection{{Multi-relational Temporal Graph Benchmarking}}\label{sec:relwork_benchmarking}
The Open Graph Benchmark (OGB)~\cite{Hu2020ogb} serves as a comprehensive benchmarking suite for static and multi-relational graphs, yet it lacks support for temporal graphs. Addressing this gap, a recent contribution by~\cite{Huang2023tgb} introduced the Temporal Graph Benchmark (TGB), tailored specifically for temporal graph learning but not featuring multi-relational graphs. 
Further, \cite{gravina2024benchmarks} conduct a detailed performance comparison for deep learning methods for dynamic graphs.

While efforts like~\cite{gastinger2023eval} have highlighted evaluation inconsistencies in TKG, their study focuses on above described smaller-scale datasets and it does not present a comprehensive evaluation framework. Moreover, recent findings by~\cite{gastinger2024baselines} reveal that a simple heuristic baseline outperforms existing methods on select datasets, and thus underscore the necessity for comparison with baselines. %r.
Notably, no existing work is dedicated to evaluating Temporal Heterogeneous Graphs (THG) \todo{double-check}.

In summary, despite the publication of diverse methods in recent years, the field, with evaluations predominantly conducted on small-scale datasets and limited time ranges, lacks a unified benchmarking framework for TKG or THG as well as a set of large-scale datasets. Our work aims to address these challenges.

%


==> chapters/x0_checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{We discuss Limitations in Section~\ref{app:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss potential negative impacts in Appendix~\ref{app:neg_impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{The authors have carefully reviewed the guidelines and made their best to comply with that.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We do not include any theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We do not include any theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include a link to a GitHub repository with code to reproduce the experimental results in Section~\ref{sec:introduction}, along with the link to the \name website with additional instructions and documentation. Please check Section~\ref{sec:experiments} for experiment description and results, Section~\ref{sec:datasets} for dataset description, and Appendix~\ref{sec:app_expdetails} for more experimental details.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All of these details can be found in Section~\ref{sec:experiments}, Appendix~\ref{sec:app_expdetails}, and Appendix~\ref{app:hyperparam} for the hyperparameters.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the average performance and the standard deviation across 5 runs for all non-deterministic methods. Please find the results in Section~\ref{sec:experiments}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details are in Appendix~\ref{sec:comp_resources}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{The original research are cited in Section~\ref{sec:datasets} and the links to datasets are presented in Appendix~\ref{app:datasetdoc}.}
  \item Did you mention the license of the assets?
    \answerYes{We discuss the dataset licenses in Appendix~\ref{app:datasetdoc}. }
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The dataset download links can be found in Appendix~\ref{app:datasetdoc}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We provide information on dataset sources in Appendix~\ref{app:datasetdoc}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We have anonymized the dataset where necessary to eliminate any personally identifiable information.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We have not used crowdsourcing or conducted research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We have not used crowdsourcing or conducted research with human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We have not used crowdsourcing or conducted research with human subjects.}
\end{enumerate}

\end{enumerate}

\newpage

%

